Enhanced Multi-Resolution Analysis for Multi-Dimensional Data Utilizing Line Filtering Techniques

In this article we introduce Line Smoothness-Increasing Accuracy-Conserving Multi-Resolution Analysis\linebreak (LSIAC-MRA). This is a procedure for exploiting convolution kernel post-processors for obtaining more accurate multi-dimensional multi-resolution analysis (MRA) in terms of error reduction. This filtering-projection tool allows for the transition of data between different resolutions while simultaneously decreasing errors in the fine grid approximation. It specifically allows for defining detail multi-wavelet coefficients when translating coarse data onto finer meshes. These coefficients are usually not defined in such cases. We show how to analytically evaluate the resulting convolutions and express the filtered approximation in a new basis. This is done by combining the filtering procedure with projection operators that allow for computational implementation of this scale transition procedure. Further, this procedure can be applied to piecewise constant approximations to functions, as it provides error reduction. We demonstrate the effectiveness of this technique in two and three dimensions.

==> Refinement_Error_Tables/2D_L-SIAC_Error_Tables/2D_L-SIAC_IC=1.tex <==
\begin{table}[hbt!]\centering
\small
 \caption{\label{tab:2DLSIACIC1}Table of $L^2$ and $L^{\infty}$ errors for initial condition $u(x,y)=\sin(2\pi x)\sin(2\pi y) $ on a series of {three} meshes using the \textbf{2D L-SIAC} filter. Notice that performing the enhancement procedure once causes a on\text{e-}time reduction in errors. Applying the enhancement procedure with each mesh refinement continues to reduce the errors.}
        \label{tab:2D_LSIAC_IC=1}
\begin{tabular}{|c||cc|cc|cc|}  
\hline &\multicolumn{2}{c|}{\textbf{Projection Error}}&\multicolumn{2}{c|}{\textbf{Enhanced Once}} &\multicolumn{2}{c|}{\textbf{Enhanced Each Refinement}}\\ \hline \textbf{N}& \multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{|c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}\\ \hline  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^0$}}\\ \hline$35$	&	$3.66e-02$	&	$8.81e-02$	&	$3.66e-02$	&	$8.81e-02$	&	$3.66e-02$	&	$8.81e-02$\\
	\hline
$70$	&	$3.66e-02$	&	$8.81e-02$	&	$1.86e-02$	&	$4.80e-02$	&	$1.86e-02$	&	$4.80e-02$\\
	\hline
$140$	&	$3.66e-02$	&	$8.81e-02$	&	$1.86e-02$	&	$4.80e-02$	&	$1.00e-02$	&	$2.67e-02$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^1$}}\\ \hline$35$	&	$8.49e-04$	&	$5.10e-03$	&	$8.49e-04$	&	$5.10e-03$	&	$8.49e-04$	&	$5.10e-03$\\
	\hline
$70$	&	$8.49e-04$	&	$5.10e-03$	&	$2.16e-04$	&	$1.18e-03$	&	$2.16e-04$	&	$1.18e-03$\\
	\hline
$140$	&	$8.49e-04$	&	$5.10e-03$	&	$2.16e-04$	&	$1.18e-03$	&	$6.43e-05$	&	$2.59e-04$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^2$}}\\ \hline$35$	&	$1.29e-05$	&	$4.63e-05$	&	$1.29e-05$	&	$4.63e-05$	&	$1.29e-05$	&	$4.63e-05$\\
	\hline
$70$	&	$1.29e-05$	&	$4.63e-05$	&	$1.72e-06$	&	$6.86e-06$	&	$1.72e-06$	&	$6.86e-06$\\
	\hline
$140$	&	$1.29e-05$	&	$4.63e-05$	&	$1.72e-06$	&	$6.86e-06$	&	$6.17e-07$	&	$1.97e-06$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^3$}}\\ \hline$35$	&	$1.46e-07$	&	$1.03e-06$	&	$1.46e-07$	&	$1.03e-06$	&	$1.46e-07$	&	$1.03e-06$\\
	\hline
$70$	&	$1.46e-07$	&	$1.03e-06$	&	$1.48e-08$	&	$6.90e-08$	&	$1.48e-08$	&	$6.90e-08$\\
	\hline
$140$	&	$1.46e-07$	&	$1.03e-06$	&	$1.48e-08$	&	$6.90e-08$	&	$1.14e-08$	&	$1.86e-08$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^4$}}\\ \hline$35$	&	$1.31e-09$	&	$5.04e-09$	&	$1.31e-09$	&	$5.04e-09$	&	$1.31e-09$	&	$5.04e-09$\\
	\hline
$70$	&	$1.31e-09$	&	$5.04e-09$	&	$2.70e-10$	&	$5.46e-10$	&	$2.70e-10$	&	$5.46e-10$\\
	\hline
$140$	&	$1.31e-09$	&	$5.04e-09$	&	$2.70e-10$	&	$5.46e-10$	&	$2.66e-10$	&	$3.90e-10$\\
	\hline
\end{tabular} 
\end{table} 

==> Refinement_Error_Tables/2D_L-SIAC_Error_Tables/2D_L-SIAC_IC=2.tex <==
\begin{table}[hbt!]\centering
  \small
  \caption{\label{tab:2DLSIACIC2}Table of $L^2$ and $L^{\infty}$ errors for initial condition $u(x,y)=\sin(2\pi (x +y)) $ on a series of {three} meshes using the \textbf{2D L-SIAC} filter. Notice that performing the enhancement procedure once causes a on\text{e-}time reduction in errors. Applying the enhancement procedure with each mesh refinement continues to reduce the errors.}
          \label{tab:2D_LSIAC_IC=2}
\begin{tabular}{|c||cc|cc|cc|}  
\hline &\multicolumn{2}{c|}{\textbf{Projection Error}}&\multicolumn{2}{c|}{\textbf{Enhanced Once}} &\multicolumn{2}{c|}{\textbf{Enhanced Each Refinement}}\\ \hline \textbf{N}& \multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{|c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}\\ \hline  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^0$}}\\ \hline$35$	&	$5.18e-02$	&	$1.76e-01$	&	$5.18e-02$	&	$1.76e-01$	&	$5.18e-02$	&	$1.76e-01$\\
	\hline
$70$	&	$5.18e-02$	&	$1.76e-01$	&	$2.60e-02$	&	$8.70e-02$	&	$2.60e-02$	&	$8.70e-02$\\
	\hline
$140$	&	$5.18e-02$	&	$1.76e-01$	&	$2.60e-02$	&	$8.70e-02$	&	$1.35e-02$	&	$4.26e-02$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^1$}}\\ \hline$35$	&	$1.20e-03$	&	$5.10e-03$	&	$1.20e-03$	&	$5.10e-03$	&	$1.20e-03$	&	$5.10e-03$\\
	\hline
$70$	&	$1.20e-03$	&	$5.10e-03$	&	$3.02e-04$	&	$1.20e-03$	&	$3.02e-04$	&	$1.20e-03$\\
	\hline
$140$	&	$1.20e-03$	&	$5.10e-03$	&	$3.02e-04$	&	$1.20e-03$	&	$7.81e-05$	&	$2.71e-04$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^2$}}\\ \hline$35$	&	$1.82e-05$	&	$8.68e-05$	&	$1.82e-05$	&	$8.68e-05$	&	$1.82e-05$	&	$8.68e-05$\\
	\hline
$70$	&	$1.82e-05$	&	$8.68e-05$	&	$2.30e-06$	&	$9.77e-06$	&	$2.30e-06$	&	$9.77e-06$\\
	\hline
$140$	&	$1.82e-05$	&	$8.68e-05$	&	$2.30e-06$	&	$9.77e-06$	&	$3.77e-07$	&	$1.23e-06$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^3$}}\\ \hline$35$	&	$2.06e-07$	&	$1.03e-06$	&	$2.06e-07$	&	$1.03e-06$	&	$2.06e-07$	&	$1.03e-06$\\
	\hline
$70$	&	$2.06e-07$	&	$1.03e-06$	&	$1.32e-08$	&	$5.34e-08$	&	$1.32e-08$	&	$5.34e-08$\\
	\hline
$140$	&	$2.06e-07$	&	$1.03e-06$	&	$1.32e-08$	&	$5.34e-08$	&	$1.55e-09$	&	$4.07e-09$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^4$}}\\ \hline$35$	&	$1.86e-09$	&	$9.39e-09$	&	$1.86e-09$	&	$9.39e-09$	&	$1.86e-09$	&	$9.39e-09$\\
	\hline
$70$	&	$1.86e-09$	&	$9.39e-09$	&	$6.20e-11$	&	$2.23e-10$	&	$6.20e-11$	&	$2.23e-10$\\
	\hline
$140$	&	$1.86e-09$	&	$9.39e-09$	&	$6.20e-11$	&	$2.23e-10$	&	$4.62e-12$	&	$1.41e-11$\\
	\hline
\end{tabular} 
\end{table} 

==> Refinement_Error_Tables/2D_L-SIAC_Error_Tables/2D_L-SIAC_IC=3.tex <==
\begin{table}[hbt!]\centering
  \small
  \caption{\label{tab:2DLSIACIC3}Table of $L^2$ and $L^{\infty}$ errors for initial condition $u(x,y)=\sin(2\pi (x +y)) $ on a series of {three} meshes using the \textbf{2D L-SIAC} filter. Notice that performing the enhancement procedure once causes a on\text{e-}time reduction in errors. Applying the enhancement procedure with each mesh refinement continues to reduce the errors.}
          \label{tab:2D_LSIAC_IC=3}
\begin{tabular}{|c||cc|cc|cc|}  
\hline &\multicolumn{2}{c|}{\textbf{Projection Error}}&\multicolumn{2}{c|}{\textbf{Enhanced Once}} &\multicolumn{2}{c|}{\textbf{Enhanced Each Refinement}}\\ \hline \textbf{N}& \multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c }{\textbf{$L^{\infty}$-Error}}&\multicolumn{1}{|c }{\textbf{$L^2$-Error}}&\multicolumn{1}{c| }{\textbf{$L^{\infty}$-Error}}\\ \hline  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^{\mathbf{0}}$}}\\ \hline$\mathbf{35}$	&	$5.18e-02$	&	$1.76e-01$	&	$5.18e-02$	&	$1.76e-01$	&	$5.18e-02$	&	$1.76e-01$\\
	\hline
$\mathbf{70}$	&	$5.18e-02$	&	$1.76e-01$	&	$2.65e-02$	&	$8.73e-02$	&	$2.65e-02$	&	$8.73e-02$\\
	\hline
$\mathbf{140}$	&	$5.18e-02$	&	$1.76e-01$	&	$2.65e-02$	&	$8.73e-02$	&	$1.50e-02$	&	$4.34e-02$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^{\mathbf{1}}$}}\\ \hline$\mathbf{35}$	&	$1.20e-03$	&	$5.10e-03$	&	$1.20e-03$	&	$5.10e-03$	&	$1.20e-03$	&	$5.10e-03$\\
	\hline
$\mathbf{70}$	&	$1.20e-03$	&	$5.10e-03$	&	$3.11e-04$	&	$1.15e-03$	&	$3.11e-04$	&	$1.15e-03$\\
	\hline
$\mathbf{140}$	&	$1.20e-03$	&	$5.10e-03$	&	$3.11e-04$	&	$1.15e-03$	&	$1.04e-04$	&	$2.47e-04$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^{\mathbf{2}}$}}\\ \hline$\mathbf{35}$	&	$1.82e-05$	&	$8.68e-05$	&	$1.82e-05$	&	$8.68e-05$	&	$1.82e-05$	&	$8.68e-05$\\
	\hline
$\mathbf{70}$	&	$1.82e-05$	&	$8.68e-05$	&	$2.59e-06$	&	$1.05e-05$	&	$2.59e-06$	&	$1.05e-05$\\
	\hline
$\mathbf{140}$	&	$1.82e-05$	&	$8.68e-05$	&	$2.59e-06$	&	$1.05e-05$	&	$1.20e-06$	&	$3.14e-06$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^{\mathbf{3}}$}}\\ \hline$\mathbf{35}$	&	$2.06e-07$	&	$1.03e-06$	&	$2.06e-07$	&	$1.03e-06$	&	$2.06e-07$	&	$1.03e-06$\\
	\hline
$\mathbf{70}$	&	$2.06e-07$	&	$1.03e-06$	&	$2.67e-08$	&	$8.50e-08$	&	$2.67e-08$	&	$8.50e-08$\\
	\hline
$\mathbf{140}$	&	$2.06e-07$	&	$1.03e-06$	&	$2.67e-08$	&	$8.50e-08$	&	$2.29e-08$	&	$3.52e-08$\\
	\hline
  &\multicolumn{6}{c|}{\textbf{$\mathbb{P}^{\mathbf{4}}$}}\\ \hline$\mathbf{35}$	&	$1.86e-09$	&	$9.39e-09$	&	$1.86e-09$	&	$9.39e-09$	&	$1.86e-09$	&	$9.39e-09$\\
	\hline
$\mathbf{70}$	&	$1.86e-09$	&	$9.39e-09$	&	$5.36e-10$	&	$9.05e-10$	&	$5.36e-10$	&	$9.05e-10$\\
	\hline
$\mathbf{140}$	&	$1.86e-09$	&	$9.39e-09$	&	$5.36e-10$	&	$9.05e-10$	&	$5.32e-10$	&	$7.76e-10$\\
	\hline
\end{tabular} 
\end{table} 

==> Refinement_Error_Tables/3D_L-SIAC_Error_Tables/3D_L-SIAC_IC=3.tex <==
\begin{table}[hbt!]\centering
\small
 \caption{\label{tab:3DLSIACIC3}Table of $L^2$ and $L^{\infty}$ errors for initial condition $u(x,y,z)=\sin(2\pi (x+y+z)) $ on a series of three meshes using the \textbf{3D L-SIAC} filter.}
\begin{tabular}{|c||cc|cc|cc|} 
\hline &\multicolumn{2}{c|}{\textbf{Projection Error}}&\multicolumn{2}{c|}{\textbf{Enhanced Once}} &\multicolumn{2}{c|}{\textbf{Enhanced Each Refinement}}\\ \hline $\mathbf{N}$& \multicolumn{1}{c }{$\mathbf{L^2}$\textbf{-Error}}&\multicolumn{1}{c| }{$\mathbf{L^{\infty}}$\textbf{-Error}}&\multicolumn{1}{c }{$\mathbf{L^2}$\textbf{-Error}}&\multicolumn{1}{c }{$\mathbf{L^{\infty}}$\textbf{-Error}}&\multicolumn{1}{|c }{$\mathbf{L^2}$\textbf{-Error}}&\multicolumn{1}{c| }{$\mathbf{L^{\infty}}$\textbf{-Error}}\\ \hline  &\multicolumn{6}{c|}{$\mathbf{\mathbb{P}^0}$}\\ \hline$\mathbf{15}$	&	$1.47e-01$	&	$6.05e-01$	&	$1.47e-01$	&	$6.05e-01$	&	$1.47e-01$	&	$6.05e-01$\\
	\hline
$\mathbf{30}$	&	$1.47e-01$	&	$6.05e-01$	&	$9.53e-02$	&	$3.19e-01$	&	$9.53e-02$	&	$3.19e-01$\\
	\hline
$\mathbf{60}$	&	$1.47e-01$	&	$6.05e-01$	&	$9.53e-02$	&	$3.19e-01$	&	$8.60e-02$	&	$1.91e-01$\\
	\hline
  &\multicolumn{6}{c|}{$\mathbf{\mathbb{P}^1}$}\\ \hline$\mathbf{15}$	&	$7.99e-03$	&	$4.20e-02$	&	$7.99e-03$	&	$4.20e-02$	&	$7.99e-03$	&	$4.20e-02$\\
	\hline
$\mathbf{30}$	&	$7.99e-03$	&	$4.20e-02$	&	$7.99e-03$	&	$1.65e-02$	&	$7.99e-03$	&	$1.65e-02$\\
	\hline
$\mathbf{60}$	&	$7.99e-03$	&	$4.20e-02$	&	$7.99e-03$	&	$1.65e-02$	&	$8.19e-03$	&	$1.36e-02$\\
	\hline
\end{tabular} 
\end{table} 

==> Sections_LSIAC/2D_LSIAC_algorithm.tex <==
\begin{algorithm}
\caption{Calculate $u^f$ from $u$ using L-SIAC kernel}\label{alg:LSIAC}

\begin{algorithmic}[1]

 \State \textbf{Input:}\text{ Number of elements in one direction $N$, and polynomial degree $p$.}\;
    
  \State \textbf{Output:}\text{ Fine mesh modal coefficients $u^f$}\;\\
  
  \State \%  \text{Compute modal projection on coarse mesh}
  \State  $u=\text{Initialize}(N,p,\Omega,u_0)$\;     \\

\State   \% \text{Compute projection matrices by region}\;
  \State  $\hphantom{[P1BL,P1BM,P1BR]}\mathllap{[P1TL,P1TM,P1TR]}\phantom{]}=\text{ProjMatrixL}(N,p,Q1T)$\;
  \State  $\hphantom{[[P1BL,P1BM,P1BR]}\mathllap{[P1BL,P1BM,P1BR]}=\text{ProjMatrixL}(N,p,Q1B)$\;
  \State  $\hphantom{[P1BL,P1BM,P1BR]}\mathllap{[P2TL,P2TM,P2TR]}\phantom{]}=\text{ProjMatrixL}(N,p,Q2T)$\;
 \State   $\hphantom{[P1BL,P1BM,P1BR]}\mathllap{[P3TL,P3TM,P3TR]}\phantom{]}=\text{ProjMatrixL}(N,p,Q3T)$\;
  \State  $\hphantom{[[P1BL,P1BM,P1BR]}\mathllap{[P3BL,P3BM,P3BR]}=\text{ProjMatrixL}(N,p,Q3B)$\;
  \State  $\hphantom{[[P1BL,P1BM,P1BR]}\mathllap{[P4BL,P4BM,P4BR]}=\text{ProjMatrixL}(N,p,Q4B)$\;\\
    
    \State \% \text{Loop through mesh elements}\;
\For{$i\gets 1, N$}
    \For{$j\gets 1, {N}$}   \\
    
    
   \State \% \text{Construct filtering/sifting matrices}\;
    
 \State   $\hphantom{Kn1n1}\mathllap{K11}\phantom{nn}=\text{FiltMatrixL}(p,1,1,i,j)$\;
\State    $\hphantom{Kn1n1}\mathllap{K01}\phantom{nn}=\text{FiltMatrixL}(p,0,1,i,j)$\;
 \State   $\hphantom{Kn1n1}\mathllap{K10}\phantom{nn}=\text{FiltMatrixL}(p,1,0,i,j)$\; 
 \State   $\hphantom{Kn1n1}\mathllap{K00}\phantom{nn}=\text{FiltMatrixL}(p,0,0,i,j)$\; 
 \State   $\hphantom{nKn1n1}\mathllap{Kn10}\phantom{n}=\text{FiltMatrixL}(p,-1,0,i,j)$\; 
\State    $\hphantom{nKn1n1}\mathllap{K0n1}\phantom{n}=\text{FiltMatrixL}(p,0,-1,i,j)$\; 
 \State   $\hphantom{nnKn1n1}\mathllap{Kn1n1}=\text{FiltMatrixL}(p,-1,-1,i,j)$\; \\
    
     \State \% \text{Compute local fine mesh coefficients}\;
   \State $u^f_{tensor}(:,2i,2j)=$
   \newline \hspace*{7em}$((P1TL+P1BL)*K00+$
   \newline \hspace*{7em} $(P1TR+P1BR)*K11+$
   \newline \hspace*{7em}$(P1TM*K01+P1BM*K10)*u$\; 

  \State  $u^f_{tensor}(:,2i-1,2j)=$
  \newline \hspace*{7em}$(P2L*Kn10+P2M*K00+P2R*K01)*u$\;
    
 \State   $u^f_{tensor}(:,2i-1,2j-1)=$
 \newline \hspace*{7em}$((P3TL+P3BL)*Kn1n1+$
  \newline \hspace*{7em}$(P3TR+P3BR)*K00+$
 \newline \hspace*{7em} $P3TM*Kn10+P3BM*K0n1)*u$\; 

  \State  $u^f_{tensor}(:,2i,2j-1)=$
  \newline \hspace*{7em}$(P4L*K0n1+P4M*K00+P4R*K10)*u$\;
        
    \EndFor
\EndFor
\\
      \State \% \text{Reshape fine modal array into original array form}\;
   \State  $u^f=\text{ReshapeArray}(p,N,u^f_{tensor})$\;
          \end{algorithmic}

\end{algorithm}


